BIRDTurk: Adaptation of the BIRD Text-to-SQL Dataset to Turkish

Text-to-SQL systems have achieved strong performance on English benchmarks, yet their behavior in morphologically rich, low-resource languages remains largely unexplored. We introduce BIRDTurk, the first Turkish adaptation of the BIRD benchmark, constructed through a controlled translation pipeline that adapts schema identifiers to Turkish while strictly preserving the logical structure and execution semantics of SQL queries and databases. Translation quality is validated on a sample size determined by the Central Limit Theorem to ensure 95% confidence, achieving 98.15% accuracy on human-evaluated samples. Using BIRDTurk, we evaluate inference-based prompting, agentic multi-stage reasoning, and supervised fine-tuning. Our results reveal that Turkish introduces consistent performance degradation, driven by both structural linguistic divergence and underrepresentation in LLM pretraining, while agentic reasoning demonstrates stronger cross-lingual robustness. Supervised fine-tuning remains challenging for standard multilingual baselines but scales effectively with modern instruction-tuned models. BIRDTurk provides a controlled testbed for cross-lingual Text-to-SQL evaluation under realistic database conditions. We release the training and development splits to support future research.

==> acl_latex <==
@book{Aho:72,
    author  = {Alfred V. Aho and Jeffrey D. Ullman},
    title   = {The Theory of Parsing, Translation and Compiling},
    year    = "1972",
    volume  = "1",
    publisher = {Prentice-Hall},
    address = {Englewood Cliffs, NJ}
}

@book{APA:83,
    author  = {{American Psychological Association}},
    title   = {Publications Manual},
    year    = "1983",
    publisher = {American Psychological Association},
    address = {Washington, DC}
}

@article{Chandra:81,
	author = {Ashok K. Chandra and Dexter C. Kozen and Larry J. Stockmeyer},
	year = "1981",
	title = {Alternation},
	journal = {Journal of the Association for Computing Machinery},
	volume = "28",
	number = "1",
	pages = "114--133",
	doi = "10.1145/322234.322243",
}

@inproceedings{andrew2007scalable,
  title={Scalable training of {L1}-regularized log-linear models},
  author={Andrew, Galen and Gao, Jianfeng},
  booktitle={Proceedings of the 24th International Conference on Machine Learning},
  pages={33--40},
  year={2007},
}

@book{Gusfield:97,
    author  = {Dan Gusfield},
    title   = {Algorithms on Strings, Trees and Sequences},
    year    = "1997",
    publisher = {Cambridge University Press},
    address = {Cambridge, UK}
}

@article{rasooli-tetrault-2015,
    author    = {Mohammad Sadegh Rasooli and Joel R. Tetreault},
    title     = {Yara Parser: {A} Fast and Accurate Dependency Parser},
    journal   = {Computing Research Repository},
    volume    = {arXiv:1503.06733},
    year      = {2015},
    url       = {http://arxiv.org/abs/1503.06733},
    note    = {version 2}
}

@article{Ando2005,
	Acmid = {1194905},
	Author = {Ando, Rie Kubota and Zhang, Tong},
	Issn = {1532-4435},
	Issue_Date = {12/1/2005},
	Journal = {Journal of Machine Learning Research},
	Month = dec,
	Numpages = {37},
	Pages = {1817--1853},
	Publisher = {JMLR.org},
	Title = {A Framework for Learning Predictive Structures from Multiple Tasks and Unlabeled Data},
	Volume = {6},
	Year = {2005}
}

@article{oflazer1994two,
  title={Two-level description of Turkish morphology},
  author={Oflazer, Kemal},
  journal={Literary and linguistic computing},
  volume={9},
  number={2},
  pages={137--148},
  year={1994},
  publisher={Oxford University Press}
}

@article{eryigit2008dependency,
  title={Dependency parsing of Turkish},
  author={Eryiğit, Gülşen and Nivre, Joakim and Oflazer, Kemal},
  journal={Computational Linguistics},
  volume={34},
  number={3},
  pages={357--389},
  year={2008},
  publisher={MIT Press}
}

@article{qin2022survey,
  title={A survey on text-to-sql parsing: Concepts, methods, and future directions},
  author={Qin, Bowen and Hui, Binyuan and Wang, Lihan and Yang, Min and Li, Jinyang and others},
  journal={arXiv preprint arXiv:2208.13629},
  year={2022}
}

@inproceedings{dou2023multispider,
  title={MultiSpider: Towards Benchmarking Multilingual Text-to-SQL Semantic Parsing},
  author={Dou, Longxu and Gao, Yan and Pan, Mingyang and Wang, Dingzirui and Che, Wanxiang and Zhan, Dechen and Lou, Jian-Guang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  pages={12745--12753},
  year={2023}
}

@inproceedings{lei2025spider2,
  title     = {Spider 2.0: Evaluating Language Models on Real-World Enterprise Text-to-{SQL} Workflows},
  author    = {Lei, Fangyu and Chen, Jixuan and Ye, Yuxiao and Cao, Ruisheng and Shin, Dongchan and Su, Hongjin and Suo, Zhaoqing and Gao, Hongcheng and Hu, Wenjing and Yin, Pengcheng and others},
  booktitle = {Proceedings of the International Conference on Learning Representations (ICLR)},
  year      = {2025},
  note      = {To appear}
}

@inproceedings{finegan-dollak-etal-2018-improving,
    title = "Improving Text-to-{SQL} Evaluation Methodology",
    author = "Finegan-Dollak, Catherine  and
      Kummerfeld, Jonathan K.  and
      Zhang, Li  and
      Ramanathan, Karthik  and
      Sadasivam, Sesh  and
      Zhang, Rui  and
      Radev, Dragomir",
    editor = "Gurevych, Iryna  and
      Miyao, Yusuke",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/P18-1033/",
    doi = "10.18653/v1/P18-1033",
    pages = "351--360",
    abstract = "To be informative, an evaluation must measure how well systems generalize to realistic unseen data. We identify limitations of and propose improvements to current evaluations of text-to-SQL systems. First, we compare human-generated and automatically generated questions, characterizing properties of queries necessary for real-world applications. To facilitate evaluation on multiple datasets, we release standardized and improved versions of seven existing datasets and one new text-to-SQL dataset. Second, we show that the current division of data into training and test sets measures robustness to variations in the way questions are asked, but only partially tests how well systems generalize to new queries; therefore, we propose a complementary dataset split for evaluation of future work. Finally, we demonstrate how the common practice of anonymizing variables during evaluation removes an important challenge of the task. Our observations highlight key difficulties, and our methodology enables effective measurement of future development."
}

@inproceedings{pourreza2023din,
 author = {Pourreza, Mohammadreza and Rafiei, Davood},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {A. Oh and T. Naumann and A. Globerson and K. Saenko and M. Hardt and S. Levine},
 pages = {36339--36348},
 publisher = {Curran Associates, Inc.},
 title = {DIN-SQL: Decomposed In-Context Learning of Text-to-SQL with Self-Correction},
 url = {https://proceedings.neurips.cc/paper_files/paper/2023/file/72223cc66f63ca1aa59edaec1b3670e6-Paper-Conference.pdf},
 volume = {36},
 year = {2023}
}

@inproceedings{scholak2021picard,
  title={{PICARD}: Parsing Incrementally for Constrained Auto-Regressive Decoding from Language Models},
  author={Scholak, Torsten and Schucher, Nathan and Bahdanau, Dzmitry},
  booktitle={Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing},
  pages={9895--9901},
  year={2021},
  organization={Association for Computational Linguistics}
}

@article{raffel2020t5,
  title={Exploring the Limits of Transfer Learning with a Unified Text-to-Text Transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={Journal of Machine Learning Research},
  volume={21},
  number={140},
  pages={1--67},
  year={2020}
}

@article{hacifazlioglu2024finetuning,
  title={Fine-tuning Large Language Models for Turkish},
  author={Hacıfazlıoğlu, H. Ozan and Partovi Nia, Vahid and Kuruoğlu, Ercan},
  journal={arXiv preprint arXiv:2407.15185},
  year={2024}
}

@article{toraman2022impact,
author = {Toraman, Cagri and Yilmaz, Eyup Halit and \c{S}ahi̇nu\c{c}, Furkan and Ozcelik, Oguzhan},
title = {Impact of Tokenization on Language Models: An Analysis for Turkish},
year = {2023},
issue_date = {April 2023},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {22},
number = {4},
issn = {2375-4699},
url = {https://doi.org/10.1145/3578707},
doi = {10.1145/3578707},
journal = {ACM Trans. Asian Low-Resour. Lang. Inf. Process.},
month = mar,
articleno = {116},
numpages = {21},
keywords = {Language model, morphological analysis, tokenization, vocabulary size}
}

@inproceedings{umutlu-etal-2025-evaluating,
    title = "Evaluating the Quality of Benchmark Datasets for Low-Resource Languages: A Case Study on {T}urkish",
    author = "Umutlu, Elif Ecem  and
      Cengiz, Ayse Aysu  and
      Sever, Ahmet Kaan  and
      Erdem, Seyma  and
      Aytan, Burak  and
      Tufan, Busra  and
      Topraksoy, Abdullah  and
      Dar{\i}c{\i}, Esra  and
      Toraman, Cagri",
    editor = "Arviv, Ofir  and
      Clinciu, Miruna  and
      Dhole, Kaustubh  and
      Dror, Rotem  and
      Gehrmann, Sebastian  and
      Habba, Eliya  and
      Itzhak, Itay  and
      Mille, Simon  and
      Perlitz, Yotam  and
      Santus, Enrico  and
      Sedoc, Jo{\~a}o  and
      Shmueli Scheuer, Michal  and
      Stanovsky, Gabriel  and
      Tafjord, Oyvind",
    booktitle = "Proceedings of the Fourth Workshop on Generation, Evaluation and Metrics (GEM{\texttwosuperior})",
    month = jul,
    year = "2025",
    address = "Vienna, Austria and virtual meeting",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2025.gem-1.41/",
    pages = "471--487",
    ISBN = "979-8-89176-261-9",
    abstract = "The reliance on translated or adapted datasets from English or multilingual resources introduces challenges regarding linguistic and cultural suitability. This study addresses the need for robust and culturally appropriate benchmarks by evaluating the quality of 17 commonly used Turkish benchmark datasets. Using a comprehensive framework that assesses six criteria, both human and LLM-judge annotators provide detailed evaluations to identify dataset strengths and shortcomings.Our results reveal that 70{\%} of the benchmark datasets fail to meet our heuristic quality standards. The correctness of the usage of technical terms is the strongest criterion, but 85{\%} of the criteria are not satisfied in the examined datasets. Although LLM judges demonstrate potential, they are less effective than human annotators, particularly in understanding cultural common sense knowledge and interpreting fluent, unambiguous text. GPT-4o has stronger labeling capabilities for grammatical and technical tasks, while Llama3.3-70B excels at correctness and cultural knowledge evaluation. Our findings emphasize the urgent need for more rigorous quality control in creating and adapting datasets for low-resource languages."
}

@article{xue2021mt5,
  title={m{T}5: A Massively Multilingual Pre-trained Text-to-Text Transformer},
  author={Xue, Linting and Constant, Noah and Roberts, Adam and Kale, Mihir and Al-Rfou, Rami and Siddhant, Aditya and Barua, Aditya and Raffel, Colin},
  journal={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={483--498},
  year={2021}
}

@article{gansql2023din,
  title={DIN-SQL: Decomposed Inference for Text-to-SQL Generation},
  author={Gan, Yujian and Chen, Xinyun and others},
  journal={arXiv preprint arXiv:2304.11015},
  year={2023}
}

@inproceedings{ahia2023do,
  title={Do All Languages Cost the Same? Tokenization in the Era of Commercial {LLM}s},
  author={Ahia, Orevaoghene and Kumar, Sachin and Gonen, Hila and Jung, Kyunghyun and Tsvetkov, Yulia and Smith, Noah A.},
  booktitle={Proceedings of the 2023 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
  pages={10760--10773},
  year={2023},
  publisher={Association for Computational Linguistics}
}

@inproceedings{rust2021good,
  title={Good-Enough Reliable Information Extraction from {T}urkish Social Media Data},
  author={Rust, Phillip and AC, Saket and K{\"o}ksal, Abdullatif and Otan, Elif and Basaran, Zeynep and Soricut, Radu and Cialdea, C and Tyers, Francis M},
  booktitle={Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={1555--1568},
  year={2021}
}

@article{petrochuk2024simple,
  title={Simple and Effective Tokenization for {T}urkish},
  author={Petrochuk, Michael and Campagna, Giovanni},
  journal={arXiv preprint arXiv:2402.15843},
  year={2024}
}

@inproceedings{conneau2020unsupervised,
  title={Unsupervised Cross-lingual Representation Learning at Scale},
  author={Conneau, Alexis and Khandelwal, Kartikay and Goyal, Naman and Chaudhary, Vishrav and Wenzek, Guillaume and Guzm{\'a}n, Francisco and Grave, Edouard and Ott, Myle and Zettlemoyer, Luke and Stoyanov, Veselin},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={8440--8451},
  year={2020}
}


@article{hakkanitur2002statistical,
  title={Statistical morphological disambiguation for Turkish text},
  author={Hakkani-T{\"u}r, Dilek Z and Oflazer, Kemal and T{\"u}r, G{\"o}khan},
  journal={International Journal of Pattern Recognition and Artificial Intelligence},
  volume={16},
  number={04},
  pages={381--402},
  year={2002}
}

@inproceedings{rust2021how,
  title={How Good is Your Tokenizer? On the Monolingual Performance of Multilingual Language Models},
  author={Rust, Phillip and others},
  booktitle={Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics},
  pages={3118--3135},
  year={2021}
}

@article{toraman2026turkbench,
  title={TurkBench: A Benchmark for Evaluating Turkish Large Language Models},
  author={Toraman, Çağrı and Sever, Ahmet Kaan and Cengiz, Ayse Aysu and Arslan, Elif Ecem and Sevinç, Görkem and Birdal, Mete Mert and Güldemir, Yusuf Faruk and Kanburoğlu, Ali Buğra and Felekoğlu, Sezen and Gürlek, Osman and Kantar, Sarp and Kütük, Birsen Şahin and Tufan, Büşra and Genç, Elif and Coşkun, Serkan and Demir, Gupse Ekin and Arayıcı, Muhammed Emin and Dursun, Olgun and Gungor, Onur and Üsküdarlı, Susan and Topraksoy, Abdullah and Darıcı, Esra},
  journal={arXiv preprint arXiv:2601.07020},
  year={2026}
}


@article{codd1970relational,
  title={A relational model of data for large shared data banks},
  author={Codd, Edgar F},
  journal={Communications of the ACM},
  volume={13},
  number={6},
  pages={377--387},
  year={1970},
  publisher={ACM New York, NY, USA}
}

@article{li2014constructing,
  title={Constructing an interactive natural language interface for relational databases},
  author={Li, Fei and Jagadish, H V},
  journal={Proceedings of the VLDB Endowment},
  volume={8},
  number={1},
  pages={73--84},
  year={2014},
  publisher={VLDB Endowment}
}

@article{zhong2017seq2sql,
  title={Seq2sql: Generating structured queries from natural language using reinforcement learning},
  author={Zhong, Victor and Xiong, Caiming and Socher, Richard},
  journal={arXiv preprint arXiv:1709.00103},
  year={2017}
}

@book{feller1968introduction,
  title={An Introduction to Probability Theory and Its Applications, Vol. 1},
  author={Feller, William},
  year={1968},
  publisher={Wiley},
  address={New York},
  edition={3rd}
}

@inproceedings{yu-etal-2018-spider,
    title = "{S}pider: A Large-Scale Human-Labeled Dataset for Complex and Cross-Domain Semantic Parsing and Text-to-{SQL} Task",
    author = "Yu, Tao  and
      Zhang, Rui  and
      Yang, Kai  and
      Yasunaga, Michihiro  and
      Wang, Dongxu  and
      Li, Zifan  and
      Ma, James  and
      Li, Irene  and
      Yao, Qingning  and
      Roman, Shanelle  and
      Zhang, Zilin  and
      Radev, Dragomir",
    editor = "Riloff, Ellen  and
      Chiang, David  and
      Hockenmaier, Julia  and
      Tsujii, Jun{'}ichi",
    booktitle = "Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing",
    month = oct # "-" # nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D18-1425/",
    doi = "10.18653/v1/D18-1425",
    pages = "3911--3921",
    abstract = "We present \textit{Spider}, a large-scale complex and cross-domain semantic parsing and text-to-SQL dataset annotated by 11 college students. It consists of 10,181 questions and 5,693 unique complex SQL queries on 200 databases with multiple tables covering 138 different domains. We define a new complex and cross-domain semantic parsing and text-to-SQL task so that different complicated SQL queries and databases appear in train and test sets. In this way, the task requires the model to generalize well to both new SQL queries and new database schemas. Therefore, Spider is distinct from most of the previous semantic parsing tasks because they all use a single database and have the exact same program in the train set and the test set. We experiment with various state-of-the-art models and the best model achieves only 9.7{\%} exact matching accuracy on a database split setting. This shows that Spider presents a strong challenge for future research. Our dataset and task with the most recent updates are publicly available at \url{https://yale-lily.github.io/seq2sql/spider}."
}

@book{aho2006compilers,
  title={Compilers: Principles, Techniques, and Tools},
  author={Aho, Alfred V and Lam, Monica S and Sethi, Ravi and Ullman, Jeffrey D},
  year={2006},
  publisher={Pearson Education},
  edition={2nd}
}

@inproceedings{li2023can,
  title     = {Can {LLM} Already Serve as a Database Interface? A {BIg} Bench for Large-Scale Database Grounded Text-to-{SQL}s},
  author    = {Li, Jinyang and Hui, Binyuan and Qu, Ge and Yang, Jiaxi and Li, Binhua and Li, Bowen and Wang, Bailin and Qin, Bowen and Geng, Ruiying and Huo, Nan and others},
  booktitle = {Advances in Neural Information Processing Systems (NeurIPS)},
  volume    = {36},
  pages     = {42330--42357},
  year      = {2023}
}

@inproceedings{price-1990-evaluation,
    title = "Evaluation of Spoken Language Systems: the {ATIS} Domain",
    author = "Price, P. J.",
    booktitle = "Speech and Natural Language: Proceedings of a Workshop Held at Hidden Valley, {P}ennsylvania, June 24-27,1990",
    year = "1990",
    url = "https://aclanthology.org/H90-1020/"
}



@inproceedings{zelle1996learning,
  title     = {Learning to parse database queries using inductive logic programming},
  author    = {Zelle, John M. and Mooney, Raymond J.},
  booktitle = {Proceedings of the Thirteenth National Conference on Artificial Intelligence (AAAI)},
  volume    = {2},
  pages     = {1050--1055},
  year      = {1996},
  publisher = {AAAI Press},
  address   = {Portland, Oregon}
}

@inproceedings{min-etal-2019-pilot,
    title = "A Pilot Study for {C}hinese {SQL} Semantic Parsing",
    author = "Min, Qingkai  and
      Shi, Yuefeng  and
      Zhang, Yue",
    editor = "Inui, Kentaro  and
      Jiang, Jing  and
      Ng, Vincent  and
      Wan, Xiaojun",
    booktitle = "Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)",
    month = nov,
    year = "2019",
    address = "Hong Kong, China",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D19-1377/",
    doi = "10.18653/v1/D19-1377",
    pages = "3652--3658",
    abstract = "The task of semantic parsing is highly useful for dialogue and question answering systems. Many datasets have been proposed to map natural language text into SQL, among which the recent Spider dataset provides cross-domain samples with multiple tables and complex queries. We build a Spider dataset for Chinese, which is currently a low-resource language in this task area. Interesting research questions arise from the uniqueness of the language, which requires word segmentation, and also from the fact that SQL keywords and columns of DB tables are typically written in English. We compare character- and word-based encoders for a semantic parser, and different embedding schemes. Results show that word-based semantic parser is subject to segmentation errors and cross-lingual word embeddings are useful for text-to-SQL."
}

@inproceedings{jose2021mrat,
  title={mRAT-SQL+GAP: A Portuguese Text-to-SQL Transformer},
  author={José, Mackson N. and Cozman, Fabio G.},
  booktitle={Proceedings of the 10th Brazilian Conference on Intelligent Systems (BRACIS)},
  pages={511--525},
  year={2021},
  publisher={Springer}
}

@inproceedings{tuan-nguyen-etal-2020-pilot,
    title = "A Pilot Study of Text-to-{SQL} Semantic Parsing for {V}ietnamese",
    author = "Tuan Nguyen, Anh  and
      Dao, Mai Hoang  and
      Nguyen, Dat Quoc",
    editor = "Cohn, Trevor  and
      He, Yulan  and
      Liu, Yang",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.364/",
    doi = "10.18653/v1/2020.findings-emnlp.364",
    pages = "4079--4085",
    abstract = "Semantic parsing is an important NLP task. However, Vietnamese is a low-resource language in this research area. In this paper, we present the first public large-scale Text-to-SQL semantic parsing dataset for Vietnamese. We extend and evaluate two strong semantic parsing baselines EditSQL (Zhang et al., 2019) and IRNet (Guo et al., 2019) on our dataset. We compare the two baselines with key configurations and find that: automatic Vietnamese word segmentation improves the parsing results of both baselines; the normalized pointwise mutual information (NPMI) score (Bouma, 2009) is useful for schema linking; latent syntactic features extracted from a neural dependency parser for Vietnamese also improve the results; and the monolingual language model PhoBERT for Vietnamese (Nguyen and Nguyen, 2020) helps produce higher performances than the recent best multilingual language model XLM-R (Conneau et al., 2020)."
}

@inproceedings{bakshandaeva-etal-2022-pauq,
    title = "{PAUQ}: Text-to-{SQL} in {R}ussian",
    author = "Bakshandaeva, Daria  and
      Somov, Oleg  and
      Dmitrieva, Ekaterina  and
      Davydova, Vera  and
      Tutubalina, Elena",
    editor = "Goldberg, Yoav  and
      Kozareva, Zornitsa  and
      Zhang, Yue",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2022",
    month = dec,
    year = "2022",
    address = "Abu Dhabi, United Arab Emirates",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2022.findings-emnlp.175/",
    doi = "10.18653/v1/2022.findings-emnlp.175",
    pages = "2355--2376",
    abstract = "Semantic parsing is an important task that allows to democratize human-computer interaction. One of the most popular text-to-SQL datasets with complex and diverse natural language (NL) questions and SQL queries is Spider. We construct and complement a Spider dataset for Russian, thus creating the first publicly available text-to-SQL dataset for this language. While examining its components - NL questions, SQL queries and databases content - we identify limitations of the existing database structure, fill out missing values for tables and add new requests for underrepresented categories. We select thirty functional test sets with different features that can be used for the evaluation of neural models' abilities. To conduct the experiments, we adapt baseline architectures RAT-SQL and BRIDGE and provide in-depth query component analysis. On the target language, both models demonstrate strong results with monolingual training and improved accuracy in multilingual scenario. In this paper, we also study trade-offs between machine-translated and manually-created NL queries. At present, Russian text-to-SQL is lacking in datasets as well as trained models, and we view this work as an important step towards filling this gap."
}

@inproceedings{almohaimeed2024ar,
  title     = {{A}r-{S}pider: {T}ext-to-{SQL} in {A}rabic},
  author    = {Almohaimeed, Saleh and Almohaimeed, Saad and Al Ghanim, Mansour and Wang, Liqiang},
  booktitle = {Proceedings of the 39th ACM/SIGAPP Symposium on Applied Computing (SAC '24)},
  pages     = {1024--1030},
  year      = {2024}
}

@article{hui2024qwen2,
  title={Qwen2.5-Coder Technical Report},
  author={Hui, Binyuan and Yang, Jian and Cui, Zeyu and Yang, Jiaxi and Liu, Dayiheng and Zhang, Lei and Liu, Tianyu and Huang, Jialong and Yu, Tong and Wang, Ganqu and others},
  journal={arXiv preprint arXiv:2409.12186},
  year={2024}
}

@article{comanici2025gemini25,
  title        = {Gemini 2.5: Pushing the Frontier with Advanced Reasoning, Multimodality, Long Context, and Next Generation Agentic Capabilities},
  author = {Google DeepMind},
  journal      = {arXiv preprint},
  year         = {2025},
  archivePrefix= {arXiv},
  eprint       = {2507.06261},
  primaryClass = {cs.CL}
}



@inproceedings{kanburoglu2023tur2sql,
  title     = {{TUR2SQL}: A Cross-Domain {T}urkish Dataset for {T}ext-to-{SQL}},
  author    = {Kanburo{\u{g}}lu, Ali Bu{\u{g}}ra and Tek, F. Boray},
  booktitle = {Proceedings of the 8th International Conference on Computer Science and Engineering (UBMK)},
  pages     = {206--211},
  year      = {2023},
  publisher = {IEEE},
  doi       = {10.1109/UBMK59864.2023.10286686}
}

@article{kanburoglu2024turspider,
  title     = {{TURSpider}: A {T}urkish {T}ext-to-{SQL} Dataset and {LLM}-Based Study},
  author    = {Kanburo{\u{g}}lu, Ali Bu{\u{g}}ra and Tek, Faik Boray},
  journal   = {IEEE Access},
  volume    = {12},
  pages     = {169379--169387},
  year      = {2024},
  publisher = {IEEE},
  doi       = {10.1109/ACCESS.2024.3498841}
}

